Heat kernel asymptotics on sequences of elliptically degenerating Riemann surfaces

This is the first of two articles in which we define an elliptically degenerating family of hyperbolic Riemann surfaces and study the asymptotic behavior of the associated spectral theory. Our study is motivated by a result from \cite{He 83}, which Hejhal attributes to Selberg, proving spectral accumulation for the family of Hecke triangle groups. In this article, we prove various results regarding the asymptotic behavior of heat kernels and traces of heat kernels for both real and complex time. In \cite{GJ 16}, we will use the results from this article and study the asymptotic behavior of numerous spectral functions through elliptic degeneration, including spectral counting functions, Selberg's zeta function, Hurwitz-type zeta functions, determinants of the Laplacian, wave kernels, spectral projections, small eigenfunctions, and small eigenvalues. The method of proof we employ follows the template set in previous articles which study spectral theory on degenerating families of finite volume Riemann surfaces (\cite{HJL 95}, \cite{HJL 97}, \cite{JoLu 97a}, and \cite{JoLu 97b}) and on degenerating families of finite volume hyperbolic three manifolds (\cite{DJ 98}). Although the types of results developed here and in \cite{GJ 16} are similar to those in existing articles, it is necessary to thoroughly present all details in the setting of elliptic degeneration in order to uncover all nuances in this setting.

==> psbox.tex <==
%% Every macro likes a little privacy...
\catcode`\@=11


                  %% -------------------------- %%


%%
%% Trying to tame the variety of \special commands for Postscript: the
%% universal internal command \PSspeci@l##1##2 takes ##1 to be the
%% filename and ##2 to be the integer scale factor*1000 (as for usual
%% TeX \scale commands)
%

\def\psfortextures{%     For TeXtures on the Macintosh
\def\PSspeci@l##1##2{%
\special{illustration ##1\space scaled ##2}}}

                          %% ----------- %%

\def\psfordvips{%      For DVIPS converter on VAX, UNIX and PC's
\def\PSspeci@l##1##2{%
\d@my=0.1bp \d@mx=\drawingwd \divide\d@mx by\d@my%
\special{PSfile=##1\space llx=\psllx\space lly=\pslly\space%
urx=\psurx\space ury=\psury\space rwi=\number\d@mx}}}

                          %% ----------- %%

%%
%% Correspond parfaitement a la doc OzTeX.
%% 
\def\psforoztex{%        For the OzTeX shareware on the Macintosh
\def\PSspeci@l##1##2{%
\special{##1 \space
      ##2 1000 div dup scale
      \putsp@ce{\number-\psllx} \putsp@ce{\number-\pslly} translate}}}
\def\putsp@ce#1{#1 }

                          %% ----------- %%

\def\psonlyboxes{%     Draft-like behaviour if none of the others works
\def\PSspeci@l##1##2{%
\at{0cm}{0cm}{\boxit{\vbox to\drawinght
  {\vss
  \hbox to\drawingwd{\at{0cm}{0cm}{\hbox{(##1)}}\hss}
  }}}}}


                  %% -------------------------- %%


%%
%% \ReadPSize{PSfilename} reads the dimensions of a PostScript drawing
%% and stores it in \drawinght(wd)
%%
\newdimen\drawinght\newdimen\drawingwd
\newdimen\psxoffset\newdimen\psyoffset
\newbox\drawingBox

\newread\epsffilein    % file to \read
\newif\ifepsffileok    % continue looking for the bounding box?
\newif\ifepsfbbfound   % success?
\newif\ifepsfverbose   % report what you're making?
\newdimen\epsfxsize    % horizontal size after scaling
\newdimen\epsfysize    % vertical size after scaling
\newdimen\epsftsize    % horizontal size before scaling
\newdimen\epsfrsize    % vertical size before scaling
\newdimen\epsftmp      % register for arithmetic manipulation
\newdimen\pspoints     % conversion factor
%%
\pspoints=1bp          % Adobe points are `big'
\epsfxsize=0pt         % Default value, means `use natural size'
\epsfysize=0pt         % ditto


\def\ReadPSize#1{
\edef\PSfilename{#1}
\global\def\epsfllx{72}
\global\def\epsflly{72}
\global\def\epsfurx{540}
\global\def\epsfury{720}
%%
%%   The first thing we need to do is to open the
%%   PostScript file, if possible.
%%
\openin\epsffilein=#1
\ifeof\epsffilein\errmessage{I couldn't open #1, will ignore it}\else
%%
%%   Okay, we got it. Now we'll scan lines until we find one that doesn't
%%   start with %. We're looking for the bounding box comment.
%%
   {\epsffileoktrue \chardef\other=12
    \def\do##1{\catcode`##1=\other}\dospecials \catcode`\ =10
    \loop
       \read\epsffilein to \epsffileline
       \ifeof\epsffilein\epsffileokfalse\else
%%
%%   We check to see if the first character is a % sign;
%%   if not, we stop reading (unless the line was entirely blank);
%%   if so, we look further and stop only if the line begins with
%%   `%%BoundingBox:'.
%%
          \expandafter\epsfaux\epsffileline:. \\%
       \fi
   \ifepsffileok\repeat
   \ifepsfbbfound\else
    \ifepsfverbose\message{No bounding box comment in #1; using defaults}\fi\fi
   }\closein\epsffilein\fi
\def\psllx{\epsfllx}\def\pslly{\epsflly}%
\def\psurx{\epsfurx}\def\psury{\epsfury}%
%% Units related by crazy factors as bp/pt=72.27/72 should be BANNED!
\drawinght=\epsfury bp%
\advance\drawinght by-\epsflly bp%
\drawingwd=\epsfurx bp%
\advance\drawingwd by-\epsfllx bp%
}

%%
%%   We still need to define the tricky \epsfaux macro. This requires
%%   a couple of magic constants for comparison purposes.
%%
{\catcode`\%=12 \global\let\epsfpercent=%\global\def\epsfbblit{%BoundingBox}}%
%%
%%   So we're ready to check for `%BoundingBox:' and to grab the
%%   values if they are found.
%%
%% \long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
%%    \def\testit{#2}\ifx\testit\epsfbblit
%%       \epsfgrab #3 . . . \\%
%%       \epsffileokfalse
%%       \global\epsfbbfoundtrue
%%    \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%
\long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
   \def\testit{#2}\ifx\testit\epsfbblit
      \epsfgrab #3 @ @ @ \\%
      \epsffileokfalse
      \global\epsfbbfoundtrue
   \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%

%%
%%   Here we grab the values and stuff them in the appropriate definitions.
%%
%% \def\epsfgrab #1 #2 #3 #4 #5\\{%
%%    \global\def\epsfllx{#1}\ifx\epsfllx\empty
%%       \epsfgrab #2 #3 #4 #5 .\\\else
%%    \global\def\epsflly{#2}%
%%    \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%
\def\epsfgrab #1 #2 #3 #4 #5\\{%
   \global\def\epsfllx{#1}\ifx\epsfllx\empty
      \epsfgrab #2 #3 #4 #5 @\\\else
   \global\def\epsflly{#2}%
   \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%


                  %% -------------------------- %%


%%
%% \psboxto(xdim;ydim){psfilename}: you specify the dimensions and
%%    TeX uniformly scales to fit the largest one. If xdim=0pt, the
%%    scale is fully determined by ydim and vice versa.
%%    Notice: psboxes are a real vboxes; couldn't take hbox otherwise all
%%    indentation and all cr's would be interpreted as spaces (hugh!).
%%
\newcount\xscale \newcount\yscale \newdimen\pscm\pscm=1cm
\newdimen\d@mx \newdimen\d@my
\let\ps@nnotation=\relax
\def\psboxto(#1;#2)#3{\vbox{
   \catcode`\:=12
   \ReadPSize{#3}
   \divide\drawingwd by 1000
   \divide\drawinght by 1000
   \d@mx=#1
   \ifdim\d@mx=0pt\xscale=1000
         \else \xscale=\d@mx \divide \xscale by \drawingwd\fi
   \d@my=#2
   \ifdim\d@my=0pt\yscale=1000
         \else \yscale=\d@my \divide \yscale by \drawinght\fi
   \ifnum\yscale=1000
         \else\ifnum\xscale=1000\xscale=\yscale
                    \else\ifnum\yscale<\xscale\xscale=\yscale\fi
              \fi
   \fi
   \divide \psxoffset by 1000\multiply\psxoffset by \xscale
   \divide \psyoffset by 1000\multiply\psyoffset by \xscale
   \global\divide\pscm by 1000
   \global\multiply\pscm by\xscale
   \multiply\drawingwd by\xscale \multiply\drawinght by\xscale
   \ifdim\d@mx=0pt\d@mx=\drawingwd\fi
   \ifdim\d@my=0pt\d@my=\drawinght\fi
\message{[#3\space [BoundingBox\string:\space\epsfllx\space\epsflly\space\epsfurx\space\epsfury]}%
\message{[scaled\space\the\xscale\string:\space\the\drawingwd\space x \the\drawinght]]}%
 \hbox to\d@mx{\hss\vbox to\d@my{\vss
   \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
      \kern-\psyoffset
      \PSspeci@l{\PSfilename}{\the\xscale}
      \vss}\hss\ps@nnotation}
   \global\ht\drawingBox=\the\drawinght
   \global\wd\drawingBox=\the\drawingwd
   \baselineskip=0pt
   \copy\drawingBox
 \vss}\hss}
  \global\psxoffset=0pt
  \global\psyoffset=0pt% These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}


                  %% -------------------------- %%

%%
%% \psboxscaled{scalefactor*1000}{PSfilename} allows to bypass the
%%   rounding errors of TeX integer divisions for situations where the
%%   TeX box should fit the original BoundingBox with a precision better
%%   than 1/1000.
%%
\def\psboxscaled#1#2{\vbox{
  \catcode`\:=12
  \ReadPSize{#2}
  \xscale=#1
  \divide\drawingwd by 1000\multiply\drawingwd by\xscale
  \divide\drawinght by 1000\multiply\drawinght by\xscale
  \divide \psxoffset by 1000\multiply\psxoffset by \xscale
  \divide \psyoffset by 1000\multiply\psyoffset by \xscale
  \global\divide\pscm by 1000
  \global\multiply\pscm by\xscale
\message{[#2\space [BoundingBox\string:\space\epsfllx\space\epsflly\space\epsfurx\space\epsfury]}%
\message{[scaled\space\the\xscale\string:\space\the\drawingwd\space x \the\drawinght]]}%
  \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
     \kern-\psyoffset
     \PSspeci@l{\PSfilename}{\the\xscale}
     \vss}\hss\ps@nnotation}
  \global\ht\drawingBox=\the\drawinght
  \global\wd\drawingBox=\the\drawingwd
  \baselineskip=0pt
  \copy\drawingBox
  \global\psxoffset=0pt
  \global\psyoffset=0pt% These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}


                  %% -------------------------- %%

%%
%%  \psbox{PSfilename} makes a TeX box having the minimal size to
%%      enclose the picture
\def\psbox#1{\psboxscaled{1000}{#1}}


                  %% -------------------------- %%

%%
%%  Annotations & Captions etc...
%%
%% \centinsert{anybox} is just a centered \midinsert, but is included as
%% people barely use the original inserts from TeX.
%%
\def\centinsert#1{\midinsert\line{\hss#1\hss}\endinsert}
\def\psannotate#1#2{\def\ps@nnotation{#2\global\let\ps@nnotation=\relax}#1}
\def\pscaption#1#2{\vbox{
   \setbox\drawingBox=#1
   \copy\drawingBox
   \vskip\baselineskip
   \vbox{\hsize=\wd\drawingBox\setbox0=\hbox{#2}
     \ifdim\wd0>\hsize
       \noindent\unhbox0\tolerance=5000
    \else\centerline{\box0}
    \fi
}}}


                  %% -------------------------- %%


%%
%% \at{#1}{#2}{#3} puts #3 at #1-higher and #2-right of the current
%%    position without moving it (to be used in annotations).
%%
\def\at#1#2#3{\setbox0=\hbox{#3}\ht0=0pt\dp0=0pt
  \rlap{\kern#1\vbox to0pt{\kern-#2\box0\vss}}}


                  %% -------------------------- %%


%%
%% \gridfill(ht;wd) makes a 1cm*1cm grid of ht by wd whose lower-left
%%   corner is the current point
%%
\newdimen\gridht \newdimen\gridwd
\def\gridfill(#1;#2){
  \setbox0=\hbox to 1\pscm
  {\vrule height1\pscm width.4pt\leaders\hrule\hfill}
  \gridht=#1
  \divide\gridht by \ht0
  \multiply\gridht by \ht0
  \advance \gridht by \ht0
  \gridwd=#2
  \divide\gridwd by \wd0
  \multiply\gridwd by \wd0
  \advance \gridwd by \wd0
  \vbox to \gridht{\leaders\hbox to\gridwd{\leaders\box0\hfill}\vfill}}


                  %% -------------------------- %%


%%
%% Useful to measure where to put annotations
%%
\def\fillinggrid{\at{0cm}{0cm}{\vbox{\gridfill(\drawinght;\drawingwd)}}}


                  %% -------------------------- %%


%%
%% \frameit{\thick}{\skip}{\anybox}
%%    draws with thickness \thick a box around \anybox, leaving \skip of
%%    blank around it. eg \frameit{0.5pt}{1pt}{\hbox{hello}}
%% \boxit{\anybox} is a shortcut.
%%
\def\frameit#1#2#3{\hbox{\vrule width#1\vbox{
  \hrule height#1\vskip#2\hbox{\hskip#2\vbox{#3}\hskip#2}%
        \vskip#2\hrule height#1}\vrule width#1}}
\def\boxit#1{\frameit{0.4pt}{0pt}{#1}}


                  %% -------------------------- %%


\catcode`\@=12 % cs containing @ are unreachable
%\catcode`\@=\active % cs containing @ are unreachable
 


